Reinvestigating the Uncovered Interest Rate Parity Puzzle via Analysis of Multivariate Tail Dependence in Currency Carry Trades

The currency carry trade is the investment strategy that involves selling low interest rate currencies in order to purchase higher interest rate currencies, thus profiting from the interest rate differentials. This is a well known financial puzzle to explain, since assuming foreign exchange risk is uninhibited and the markets have rational risk-neutral investors, then one would not expect profits from such strategies. That is uncovered interest rate parity (UIP), the parity condition in which exposure to foreign exchange risk, with unanticipated changes in exchange rates, should result in an outcome that changes in the exchange rate should offset the potential to profit from such interest rate differentials. The two primary assumptions required for interest rate parity are related to capital mobility and perfect substitutability of domestic and foreign assets. Given foreign exchange market equilibrium, the interest rate parity condition implies that the expected return on domestic assets will equal the exchange rate-adjusted expected return on foreign currency assets. However, it has been shown empirically, that investors can actually earn arbitrage profits by borrowing in a country with a lower interest rate, exchanging for foreign currency, and investing in a foreign country with a higher interest rate, whilst allowing for any losses (or gains) from exchanging back to their domestic currency at maturity. Therefore trading strategies that aim to exploit the interest rate differentials can be profitable on average. The intention of this paper is therefore to reinterpret the currency carry trade puzzle in light of heavy tailed marginal models coupled with multivariate tail dependence features in the analysis of the risk-reward for the currency portfolios with high interest rate differentials and low interest rate differentials.

==> ModellingTheMarginalDistributions_MA_14_Nov_2013_v3_0_0.tex <==
\section{Modelling the Marginal Exchange Rate Log-Returns}

% MARGINS



% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Proportion of rejections of the null hypothesis that the sample is from a log normal distribution, measured using a k-s test at the 5\% level.}
    \begin{tabular}{ccccccccccc}
    \toprule
    \textbf{Block length} & \textbf{EUR} & \textbf{TRY} & \textbf{JPY} & \textbf{GBP} & \textbf{AUD} & \textbf{CAD} & \textbf{NOK} & \textbf{CHF} & \textbf{SEK} & \textbf{MXN} \\
    \midrule
    \textbf{6 month} & 0.001 & 0.198 & 0.043 & 0.000 & 0.023 & 0.000 & 0.000 & 0.031 & 0.012 & 0.032 \\
    \textbf{Year} & 0.000 & \textbf{0.553} & 0.107 & 0.007 & 0.120 & 0.018 & 0.006 & 0.084 & 0.018 & 0.128 \\
    \midrule
          &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \textbf{Block length} & \textbf{PLN} & \textbf{MYR} & \textbf{SGD} & \textbf{INR} & \textbf{ZAR} & \textbf{NZD} & \textbf{THB} & \textbf{KRW} & \textbf{TWD} & \textbf{BRL} \\
    \midrule
    \textbf{6 month} & 0.018 & 0.494 & 0.000 & 0.234 & 0.025 & 0.012 & 0.221 & 0.130 & 0.192 & 0.086 \\
    \textbf{Year} & 0.094 & \textbf{0.651} & 0.071 & \textbf{0.549} & 0.124 & 0.113 & \textbf{0.504} & 0.350 & 0.381 & 0.403 \\
    \bottomrule
    \end{tabular}%
  \label{margin_decision}%
\end{table}%

{\bf Comment:} The goodness-of-fit ...

consider more flexible models for some currencies - GIG/NIG?



%\newpage

%% -------- MARGIN PLOTS ---------------- %%

% MU

\begin{figure}[p]
\centering
\includegraphics[width = \linewidth , height=110mm]{mu_gengamma_1}
%\caption{$\mu$ (log-scale) parameter of margins using 6 month blocks}
\label{mu_6m_1}
%\end{figure}
%\begin{figure}[p]
%\centering
\includegraphics[width = \linewidth , height=110mm]{mu_gengamma_2}
\caption{$\mu$ parameter of log generalised gamma margins using 6 month blocks}
%\label{mu_6m_2}
\end{figure}







% SIGMA

\begin{figure}[p]
\centering
\includegraphics[width = \linewidth , height=110mm]{sigma_gengamma_1}
%\caption{$\sigma$ (log-scale) parameter of margins using 6 month blocks}
\label{sigma_gengamma_1}
%\end{figure}
%\begin{figure}[p]
\centering
\includegraphics[width = \linewidth , height=110mm]{sigma_gengamma_2}
\caption{$\sigma$ parameter of log generalised gamma margins using 6 month blocks}
%\label{sigma_6m_2}
\end{figure}



% K
	
\begin{figure}[p]
\centering
\includegraphics[width = \linewidth , height=110mm]{k_gengamma_1}
%\caption{K parameter of log generalised gamma of margins using 6 month blocks}
\label{k_gengamma_1}
%\end{figure}
%\begin{figure}[p]
\centering
\includegraphics[width = \linewidth , height=110mm]{k_gengamma_2}
\caption{K parameter of log generalised gamma margins using 6 month blocks}
%\label{k_gengamma_2}
\end{figure}

